SynBody: Synthetic Dataset with Layered Human Models for 3D Human Perception and Modeling

Synthetic data has emerged as a promising source for 3D human research as it offers low-cost access to large-scale human datasets. To advance the diversity and annotation quality of human models, we introduce a new synthetic dataset, SynBody, with three appealing features: 1) a clothed parametric human model that can generate a diverse range of subjects; 2) the layered human representation that naturally offers high-quality 3D annotations to support multiple tasks; 3) a scalable system for producing realistic data to facilitate real-world tasks. The dataset comprises 1.2M images with corresponding accurate 3D annotations, covering 10,000 human body models, 1,187 actions, and various viewpoints. The dataset includes two subsets for human pose and shape estimation as well as human neural rendering. Extensive experiments on SynBody indicate that it substantially enhances both SMPL and SMPL-X estimation. Furthermore, the incorporation of layered annotations offers a valuable training resource for investigating the Human Neural Radiance Fields (NeRF).

==> figures/3_2_2_GarmentSewing.tex <==
\begin{figure}[htbp]
  \includegraphics[width=\linewidth]{images/GarmentSewing.png}
  \centering
  {(a) ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ (b)~~~~~~~}
  \caption{Garment Example. Left: garment pattern with sewing lines. Right: simulated garment under the body in canonical space.}
  \label{fig:GarmentSewing}
\end{figure}

==> figures/3_2_3_ClothAnimation.tex <==
\begin{figure}[htbp]
  \includegraphics[width=\linewidth]{images/Tailor.png}
  \caption{Synthesized Garment Animation.}
  \label{fig:GarmentAnimation}
\end{figure}

==> figures/synbody_demo.tex <==
\begin{figure*}[ht]
  \includegraphics[width=\linewidth]{images/synbody_teaser.png}
  \caption{Overview of SynBody dataset. \todo{@haiyi}}
  \label{fig:synbody_demo}
\end{figure*}

==> macros.tex <==
\usepackage{xcolor}
\usepackage{wrapfig}
\usepackage{soul}

\definecolor{yellow}{rgb}{1,1, 0.6}
\definecolor{lightyellow}{rgb}{1,1, 0.8}
\definecolor{orange}{rgb}{1, 0.8, 0.6}
\definecolor{coral}{RGB}{246,131,65}
\definecolor{pinkred}{rgb}{1, 0.6, 0.6}
\definecolor{hotpink}{RGB}{238,64,195}
\definecolor{lavender}{RGB}{207,226,243}
\definecolor{gainsboro}{RGB}{208,224,227}
\definecolor{gainsboro2}{RGB}{217,234,211}
\definecolor{blanchedalmond}{RGB}{252,229,205}

\newcommand{\missfigure}{\textcolor{red}{[F]}}
\newcommand{\misscite}{\textcolor{red}{[C]}}
\newcommand{\missref}{\textcolor{red}{[R]}}

\newcommand{\ray}[1]{{\textcolor{red}{#1}}}
\newcommand{\todo}[1]{{\textcolor{red}{(TODO: #1)}}}

\newcommand{\model}{XXXX}
\newcommand{\modelname}{XXXX\xspace}

\newcommand{\coverage}{spatial coverage\xspace}
\newcommand{\complexity}{detail complexity\xspace}
%altitude or distance
\newcommand{\altitude}{distance\xspace}
\newcommand{\altitudefull}{distance to the scene\xspace}
\newcommand{\altitudes}{distances\xspace}
\newcommand{\altitudesfull}{distances to the scene\xspace}

\newcommand{\copyrightgoogle}{\href{https://www.google.com/help/terms_maps/}{\textcopyright 2022 Google}\xspace}

==> sections/5_experiment.tex <==
\section{Experiment}
\label{sec:experiment}

\subsection{SMPL Estimation}

% image-based: HMR/SPIN/HybrIK/PARE/CLIFF
%video-based: VIBE/MEVA/DeciWatch

%\todo{@shuai}
%This section presents the adopted body model for training and evaluation of generated results, alongside the benchmarking metrics utilized for comprehensive assessments.
%Detailed results obtained from our evaluation approach on popular benchmarks will also be showcased.

\noindent\textbf{Body Model and Baselines.}
%
The experiments in this study employ the SMPL model~\cite{loper2015smpl}, a differentiable function that represents humans as 3D triangle meshes denoted by $M(\theta,\ \beta)\ \in \mathbb{R}^{6890\times3}$. This model representation comprises of pose parameters denoted by $\theta\in \mathbb{R}^{72}$ and shape parameters denoted by $\beta\in \mathbb{R}^{10}$. Our study focuses on training and evaluation of three image-based methods of HMR~\cite{kanazawa2018end}, SPIN~\cite{kolotouros2019learning}, and PARE~\cite{kocabas2021pare} and one video-based method of VIBE~\cite{kocabas2020vibe}.


\noindent\textbf{Evaluation Metrics.}
%
For evaluating 3D human pose estimation, this study employs two commonly used metrics, namely \textbf{MPJPE} (Mean Per Joint Position Error) and \textbf{PA-MPJPE} (Procrustes Aligned Mean Per Joint Position Error). The MPJPE is calculated as $L_2$ distance averaged over all joints, while PA-MPJPE aligns the predicted keypoints to match the ground-truth with the Procrustes method~\cite{Gower1975}, before computing the MPJPE between the aligned pose and ground truth. Additionally, we also calculate \textbf{PVE} (Per Vertex Error), which is the average distance between predicted and ground-truth mesh vertices.

\input{tables/smpl_baseline}

\noindent\textbf{Results on 3DPW testset.}
%
Table~\ref{tab:smpl_baseline} illustrates three main observations:
%
\textbf{(1) Training strategy.} We experiment with two training strategies, namely Blended Training (BT) and Finetuning (FT). The former train synthetic and real data jointly, while the latter forms the training in a two-stage procedure, which first trains with real data and then finetune with a combination of real and synthetic data.
Table~\ref{tab:smpl_baseline} demonstrates that no matter FT or BT applies, significant performance gain is obtained compared to training with only real data;
%
\textbf{(2) Baseline Model.} Consistent improvements are observed across different baseline models, even when the recent method~\cite{kocabas2021pare} achieves low errors, it still obtains 2.81\% and 0.9\% on MPJPE and PA-MPJPE, respectively.
%
\textbf{(3) Video-based Method.} As \name naturally consists of videos, it can also be used for training video-based approaches. Experiments on VIBE show improved results on all metrics when compared to the baseline.   
%
%The impact of SynBody on the performance of four baselines is presented in Table \ref{tab:smpl_baseline}. The evaluation results show that our SynBody data improves the accuracy of these baselines on 3DPW test set when combined with real datasets.
%
%In this study, we establish a balance between real and synthetic datasets by setting a 1:1 ratio in both the Blended Training (BT), and Finetuning (FT) phases. During FT, we utilize a total of 1e5 instances in each epoch and fine-tune a pre-trained model.
%Specifically, the study further employed BT and FT methods on HMR, resulting in performance gains of 8.3\% and 14.6\% in PA-MJPJE, respectively. In contrast, we employ all available data in BT while employing the models pre-trained on ImageNet. Moreover, the FT trained models achieve an improved performance of 8.7\% and 1.8\%, respectively, compared to the SPIN and PARE baselines. Additionally, SynBody, which is a video dataset, is also leveraged to refine the VIBE method, resulting in improved results on MPJPE and PVE when compared to the baseline approach.

\input{tables/smpl_baseline_2}
\input{figures/multiplies_of_real_data}
\input{tables/synbody_vs_agora}
\input{tables/human_nerf}

\noindent\textbf{Results on AGORA validation set.}
%
AGORA~\cite{patel2021agora}, a recent synthetic dataset, has draw more attention as its more challenging than 3DPW in terms of environmental and person-person occlusion.
%
Table \ref{tab:smpl_baseline} illustrates that training with \name exhibits remarkable improvements across methods, when compared with the baseline models in AGORA validation set.

%To ensure the comprehensiveness of our experimental results, we conduct an evaluation of the models presented in Table \ref{tab:smpl_baseline} using a separate benchmark comprised of synthetic data (AGORA~\cite{patel2021agora}). The findings of our assessment are illustrated in Table \ref{tab:smpl_baseline_2}. It is noteworthy that the performance of our models exhibits remarkable improvements when compared with the baseline models in AGORA validation set.

\noindent\textbf{The effect of data scale.}
%
%The present study aims to demonstrate the considerable advantages that SynBody's substantial size provides by performing HMR BT experiments where the amount of SynBody data is varied by multiples of Real.
As our generation system can easily scale the data size while maintaining data diversity, we conduct blended training with HMR to study the influence of synthetic data scale.
Figure~\ref{fig:multiplies} demonstrates that adding more SynBody data generally leads to better performance.
These experiments confirm that synthetic data is a valuable complement to real data and serves as a readily scalable training source to supplement the typically limited real data.

\noindent\textbf{Comparison with AGORA training set.}
%
%Furthermore, in the present study, we undertook a comparison of the FT outcomes generated by AGORA and SynBody. In order to ensure that our experiments were equitable, we randomly extracted a subset of SynBody called ``SynBody-10W'' that is comparable in size to AGORA. The results, as presented in Table~\ref{tab:synbody_agora}, unequivocally demonstrate superior outcomes from SynBody-10W in comparison to AGORA, thereby underscoring the exceptional quality of our datasets in comparison to existing resources.
%
To demonstrate the efficacy of data diversity and high-quality annotations, we sample a subset, ``SynBody-100K'', comparable in size to AGORA.
%
Results presented in Table~\ref{tab:synbody_agora} indicate that training with \name outperforms training with AGORA using three different methods.
%
The findings emphasize the significance of synthetic data's diversity and annotation quality for achieving superior performance with equivalent data volume.


% SMPL-X section
\subsection{SMPL-X Estimation}

\input{tables/smplx_baseline}

SMPL-X~\cite{pavlakos2019expressive} is an expressive human parametric model. In addition to SMPL's pose and shape parameters, SMPL-X consists of additional left and right hand pose parameters ($\theta_{lh}, \theta_{rh} \in \mathbb{R}^{15\times3}$), jaw joint rotation ($\theta_{lh} \in  \mathbb{R}^{3}$) and face expression parameters ($\phi_{f} \in \mathbb{R}^{10}$). In Table~\ref{tab:smplx_baseline}, we conduct experiments with Hand4Whole~\cite{moon2022accurate} as the base model with the Finetuning (FT) strategy on EHF~\cite{pavlakos2019expressive}, a real-captured dataset for expressive human body, hands, and face modelling. Since EHF does not provide SMPL-X parameters, we follow Hand4Whole and report vertex-based error (PVE) for respective body parts. We observe that finetuning on a converged Hand4Whole with a mixture of SynBody and real datasets leads to a significant improvements in both overall estimation and part-level estimation. We speculate that it is difficult to obtain accurate SMPL-X annotations (Hand4Whole uses COCO \cite{lin2014microsoft}, MPII \cite{andriluka20142d} and Human3.6M \cite{h36m_pami} with pseudo ground truth generated by NeuralAnnot \cite{moon2022neuralannot}). However, SynBody provides a large-scale high-quality SMPL-X labels paired with images that are rendered with diverse backgrounds and lighting conditions, which are beneficial to training a high-performing expressive human parametric model recovery.


\subsection{Human NeRF}

In this section, we benchmark popular NeRF-based methods for 3D humans on \name, validating the effectiveness and great potential of our dataset in human neural rendering. Our benchmark is built upon three perspectives according to the purpose of synthesis tasks, which can be categorized into novel view, novel pose, and novel identity.

\noindent\textbf{Methods for Benchmark.}
% 
We benchmark 5 methods in total, including the vanilla NeRF~\cite{mildenhall_nerf_2020}, NeuralBody~\cite{peng2021neural} and HumanNeRF~\cite{weng_humannerf_2022_cvpr} for novel view synthesis, AnimNeRF~\cite{peng2021animatable} for novel pose synthesis, NHP~\cite{kwon2021neural} for generalizable human NeRF (novel identity synthesis). Except NHP, all methods are trained in a person-specific manner, taking 4 views of the first 250 frames for training and the rest views and frames for evaluations.

\noindent\textbf{Evaluation Protocols.}
% 
We follow~\cite{mildenhall_nerf_2020, weng_humannerf_2022_cvpr} to evaluate all methods using three standard metrics: Peak Signal-to-Noise Ratio (PSNR), Structural SIMilarity index (SSIM), and Learned Perceptual Image Patch Similarity (LPIPS~\cite{zhang2018unreasonable}). To reach a consensus among all methods, all metrics are computed over the whole image with a black background. 

\noindent\textbf{Main Results.}
% 
Benchmark results are reported in Table \ref{tab:humannerf}. We observe that all methods achieve comparable performances as real human data on \name. Models (NeuralBody and AnimNeRF) which rely on accurate SMPL estimation and blending weights perform better on novel poses. We attribute it to our layer-wise design which offers ground truth SMPL parameters for human NeRF training. Besides, we present visualization results in Figure~\ref{fig:humannerf}, observing that the diverse motions and appearances, as well as loose garments in \name, pose further challenges in the field of neural rendering of 3D humans.

\input{figures/humannerf_vis}

==> sections/5_experiment_arxiv.tex <==
\section{Experiment}
\label{sec:experiment}

\subsection{SMPL Estimation}

% image-based: HMR/SPIN/HybrIK/PARE/CLIFF
%video-based: VIBE/MEVA/DeciWatch

%\todo{@shuai}
%This section presents the adopted body model for training and evaluation of generated results, alongside the benchmarking metrics utilized for comprehensive assessments.
%Detailed results obtained from our evaluation approach on popular benchmarks will also be showcased.

\noindent\textbf{Body Model and Baselines.}
%
The experiments in this study employ the SMPL model~\cite{loper2015smpl}, a differentiable function that represents humans as 3D triangle meshes denoted by $M(\theta,\ \beta)\ \in \mathbb{R}^{6890\times3}$. This model representation comprises of pose parameters denoted by $\theta\in \mathbb{R}^{72}$ and shape parameters denoted by $\beta\in \mathbb{R}^{10}$. Our study focuses on training and evaluation of three image-based methods of HMR~\cite{kanazawa2018end}, SPIN~\cite{kolotouros2019learning}, and PARE~\cite{kocabas2021pare} and one video-based method of VIBE~\cite{kocabas2020vibe}.


\noindent\textbf{Evaluation Metrics.}
%
For evaluating 3D human pose estimation, this study employs two commonly used metrics, namely \textbf{MPJPE} (Mean Per Joint Position Error) and \textbf{PA-MPJPE} (Procrustes Aligned Mean Per Joint Position Error). The MPJPE is calculated as $L_2$ distance averaged over all joints, while PA-MPJPE aligns the predicted keypoints to match the ground-truth with the Procrustes method~\cite{Gower1975}, before computing the MPJPE between the aligned pose and ground truth. Additionally, we also calculate \textbf{PVE} (Per Vertex Error), which is the average distance between predicted and ground-truth mesh vertices.

\input{tables/smpl_baseline}

\noindent\textbf{Results on 3DPW testset.}
%
Table~\ref{tab:smpl_baseline} illustrates three main observations:
%
\textbf{(1) Training strategy.} We experiment with two training strategies, namely Blended Training (BT) and Finetuning (FT). The former train synthetic and real data jointly, while the latter forms the training in a two-stage procedure, which first trains with real data and then finetune with a combination of real and synthetic data.
Table~\ref{tab:smpl_baseline} demonstrates that no matter FT or BT applies, significant performance gain is obtained compared to training with only real data;
%
\textbf{(2) Baseline Model.} Consistent improvements are observed across different baseline models, even when the recent method~\cite{kocabas2021pare} achieves low errors, it still obtains 2.81\% and 0.9\% on MPJPE and PA-MPJPE, respectively.
%
\textbf{(3) Video-based Method.} As \name naturally consists of videos, it can also be used for training video-based approaches. Experiments on VIBE show improved results on all metrics when compared to the baseline.   
%
%The impact of SynBody on the performance of four baselines is presented in Table \ref{tab:smpl_baseline}. The evaluation results show that our SynBody data improves the accuracy of these baselines on 3DPW test set when combined with real datasets.
%
%In this study, we establish a balance between real and synthetic datasets by setting a 1:1 ratio in both the Blended Training (BT), and Finetuning (FT) phases. During FT, we utilize a total of 1e5 instances in each epoch and fine-tune a pre-trained model.
%Specifically, the study further employed BT and FT methods on HMR, resulting in performance gains of 8.3\% and 14.6\% in PA-MJPJE, respectively. In contrast, we employ all available data in BT while employing the models pre-trained on ImageNet. Moreover, the FT trained models achieve an improved performance of 8.7\% and 1.8\%, respectively, compared to the SPIN and PARE baselines. Additionally, SynBody, which is a video dataset, is also leveraged to refine the VIBE method, resulting in improved results on MPJPE and PVE when compared to the baseline approach.

\input{tables/smpl_baseline_2}
\input{figures/multiplies_of_real_data}
\input{tables/synbody_vs_agora}
\input{tables/human_nerf}

\noindent\textbf{Results on AGORA validation set.}
%
AGORA~\cite{patel2021agora}, a recent synthetic dataset, has draw more attention as its more challenging than 3DPW in terms of environmental and person-person occlusion.
%
Table \ref{tab:smpl_baseline} illustrates that training with \name exhibits remarkable improvements across methods, when compared with the baseline models in AGORA validation set.

%To ensure the comprehensiveness of our experimental results, we conduct an evaluation of the models presented in Table \ref{tab:smpl_baseline} using a separate benchmark comprised of synthetic data (AGORA~\cite{patel2021agora}). The findings of our assessment are illustrated in Table \ref{tab:smpl_baseline_2}. It is noteworthy that the performance of our models exhibits remarkable improvements when compared with the baseline models in AGORA validation set.

\noindent\textbf{The effect of data scale.}
%
%The present study aims to demonstrate the considerable advantages that SynBody's substantial size provides by performing HMR BT experiments where the amount of SynBody data is varied by multiples of Real.
As our generation system can easily scale the data size while maintaining data diversity, we conduct blended training with HMR to study the influence of synthetic data scale.
Figure~\ref{fig:multiplies} demonstrates that adding more SynBody data generally leads to better performance.
These experiments confirm that synthetic data is a valuable complement to real data and serves as a readily scalable training source to supplement the typically limited real data.

\noindent\textbf{Comparison with AGORA training set.}
%
%Furthermore, in the present study, we undertook a comparison of the FT outcomes generated by AGORA and SynBody. In order to ensure that our experiments were equitable, we randomly extracted a subset of SynBody called ``SynBody-10W'' that is comparable in size to AGORA. The results, as presented in Table~\ref{tab:synbody_agora}, unequivocally demonstrate superior outcomes from SynBody-10W in comparison to AGORA, thereby underscoring the exceptional quality of our datasets in comparison to existing resources.
%
To demonstrate the efficacy of data diversity and high-quality annotations, we sample a subset, ``SynBody-10W'', comparable in size to AGORA.
%
Results presented in Table~\ref{tab:synbody_agora} indicate that training with \name outperforms training with AGORA using three different methods.
%
The findings emphasize the significance of synthetic data's diversity and annotation quality for achieving superior performance with equivalent data volume.


\subsection{Human NeRF}
%\todo{@zhaoxi}

In this section, we benchmark popular NeRF-based methods for 3D humans on \name, validating the effectiveness and great potential of our dataset in human neural rendering. Our benchmark is built upon three perspectives according to the purpose of synthesis tasks, which can be categorized into novel view, novel pose, and novel identity.

\noindent\textbf{Methods for Benchmark.}
% 
We benchmark 5 methods in total, including the vanilla NeRF~\cite{mildenhall_nerf_2020}, NeuralBody~\cite{peng2021neural} and HumanNeRF~\cite{weng_humannerf_2022_cvpr} for novel view synthesis, AnimNeRF~\cite{peng2021animatable} for novel pose synthesis, NHP~\cite{kwon2021neural} for generalizable human NeRF (novel identity synthesis). Except NHP, all methods are trained in a person-specific manner, taking 4 views of the first 250 frames for training and the rest views and frames for evaluations.

\noindent\textbf{Evaluation Protocols.}
% 
We follow~\cite{mildenhall_nerf_2020, weng_humannerf_2022_cvpr} to evaluate all methods using three standard metrics: Peak Signal-to-Noise Ratio (PSNR), Structural SIMilarity index (SSIM), and Learned Perceptual Image Patch Similarity (LPIPS~\cite{zhang2018unreasonable}). To reach a consensus among all methods, all metrics are computed over the whole image with a black background. 

\noindent\textbf{Main Results.}
% 
Benchmark results are reported in Table \ref{tab:humannerf}. We observe that all methods achieve comparable performances as real human data on \name. Models (NeuralBody and AnimNeRF) which rely on accurate SMPL estimation and blending weights perform better on novel poses. We attribute it to our layer-wise design which offers ground truth SMPL parameters for human NeRF training. Besides, we present visualization results in Figure~\ref{fig:humannerf}, observing that the diverse motions and appearances, as well as loose garments in \name, pose further challenges in the field of neural rendering of 3D humans.

\input{figures/humannerf_vis}

==> sections/6_conclusion.tex <==
\vspace{-5pt}
\section{Conclusion}
\label{sec:conclusion}
%
We present \name, a large-scale synthetic dataset that features a substantial number of subjects and high-quality 3D annotations. At the core is a clothed human model with multiple layers of representation.
%
Our experiments demonstrate the effectiveness of SynBody on both human pose and shape estimation and human NeRF.
%
Future research can leverage \name for developing and evaluating methods to predict body and cloth simultaneously.
%
Furthermore, the high controllability of synthetic dataset offers ample opportunities for further improvement, such as the incorporation of contact labels for human-scene interaction.

\noindent\textbf{Societal Impacts.}
%Despite being a synthetic dataset, \name's generation process may result in unbalanced asset usage. While hairstyles and skin color are randomly sampled, they do not exhibit any racial bias. However, the remaining assets, including body shape and clothing, may demonstrate imbalances that could introduce bias into the generated human models.
Although \name is a synthetic dataset, the assets used for its generation may be unbalanced. While hairstyles and skin color are sampled randomly, they do not result in racial bias. However, the remaining assets, such as body shape and clothing, may be imbalanced, leading to potential bias in the generated human models.

==> tables/smpl_baseline.tex <==
% % \begin{table*}[t]
% \begin{table}[htp]
%   \begin{center}
%   \caption{Training results on popular baselines with real and SynBody datasets on 3DPW Testset. ``R'' means the public academic datasets of real human and ``S'' means our SynBody data.}
%   \label{tab:smpl_baseline}
%   \resizebox{0.5\textwidth}{!}{
%   \begin{tabular}{lcllccc}
%     \toprule
%     Method  & BT/FT & Pretrained & Datasets & MPJPE & PA-MPJPE & PVE \\    
%     \midrule
    
%     HMR \cite{kanazawa2018end} & - & ImageNet & R & 112.30  & 67.50 & 141.92 \\

%     HMR & BT & ImageNet & R + S & 102.67  & 60.81  & 119.02 \\

%     HMR & FT & HMR & R + S & \textbf{95.01}  & \textbf{57.62}  & \textbf{116.10} \\

%     SPIN \cite{kolotouros2019learning} & - & ImageNet & R & 96.90  & 59.20  & 119.70 \\

%     SPIN & FT & SPIN & R + S & \textbf{84.14}  & \textbf{53.67}  & \textbf{103.79} \\

%     PARE \cite{kocabas2021pare} & - & ImageNet & R & 81.79  & 49.36  & 105.27 \\

%     PARE & FT & PARE & R + S & \textbf{78.98}  & \textbf{48.46}  & \textbf{103.86} \\

%     VIBE \cite{kocabas2020vibe} & - & HMR & R & 94.88 & \textbf{57.08}  & 108.59 \\
    
%     VIBE & BT & HMR & R + S & \textbf{90.68}  & 57.96 & \textbf{104.91} \\
    
%     \bottomrule
%   \end{tabular}
%   }
% \end{center}
% % \vspace{-0.3cm}
% \end{table}

\begin{table}[htp]
  \begin{center}
  \caption{Training results on popular baselines with real and SynBody datasets on 3DPW Testset. ``R'' means the public academic datasets of real human and ``S'' means our SynBody data.}
  \label{tab:smpl_baseline}
  \resizebox{0.48\textwidth}{!}{
  \begin{tabular}{lclccc}
    \toprule
    Method  & BT/FT & Datasets & MPJPE & PA-MPJPE & PVE \\    
    \midrule
    
    HMR \cite{kanazawa2018end} & - & R & 112.30  & 67.50 & 141.92 \\

    HMR & BT & R + S & 102.67  & 60.81  & 119.02 \\

    HMR & FT & R + S & \textbf{95.01}  & \textbf{57.62}  & \textbf{116.10} \\

    SPIN \cite{kolotouros2019learning} & - & R & 96.90  & 59.20  & 119.70 \\

    SPIN & FT & R + S & \textbf{84.14}  & \textbf{53.67}  & \textbf{103.79} \\

    PARE \cite{kocabas2021pare} & - & R & 81.79  & 49.36  & 105.27 \\

    PARE & FT & R + S & \textbf{78.98}  & \textbf{48.46}  & \textbf{103.86} \\

    VIBE \cite{kocabas2020vibe} & - & R & 94.88 & 57.08  & 108.59 \\
    
    VIBE & BT & R + S & \textbf{93.04}  & \textbf{57.00} & \textbf{107.23} \\
    
    \bottomrule
  \end{tabular}
  }
\end{center}
\vspace{-0.6cm}
\end{table}

==> tables/smplx_baseline.tex <==
\begin{table}[t]
  \begin{center}
  \caption{SMPL-X estimation with Hand4Whole~\cite{moon2022accurate} as the baseline on EHF~\cite{pavlakos2019expressive}. Finetuning with large-scale, diverse SynBody data leads to significant performance improvements. For hands, Hand4Whole reports mean value only and we report both right hand / left hand values. The metric is PVE (mm).}
  \label{tab:smplx_baseline}
  \resizebox{\linewidth}{!}{
  \begin{tabular}{lcllccccc}
    \toprule
    Method  & FT & Datasets & All & Hands & Face \\    
    \midrule
    Hand4Whole & - & R & 76.8 & 39.8 & 26.1 \\
    Hand4Whole & \checkmark & R + S & 53.5 & 37.6 / 34.8 & 14.6 \\
    \bottomrule
  \end{tabular}
  }
\end{center}
\vspace{-0.5cm}
\end{table}

